Array Folds Logic

We present an extension to the quantifier-free theory of integer arrays which allows us to express counting. The properties expressible in Array Folds Logic (AFL) include statements such as "the first array cell contains the array length," and "the array contains equally many minimal and maximal elements." These properties cannot be expressed in quantified fragments of the theory of arrays, nor in the theory of concatenation. Using reduction to counter machines, we show that the satisfiability problem of AFL is PSPACE-complete, and with a natural restriction the complexity decreases to NP. We also show that adding either universal quantifiers or concatenation leads to undecidability. AFL contains terms that fold a function over an array. We demonstrate that folding, a well-known concept from functional languages, allows us to concisely summarize loops that count over arrays, which occurs frequently in real-life programs. We provide a tool that can discharge proof obligations in AFL, and we demonstrate on practical examples that our decision procedure can solve a broad range of problems in symbolic testing and program verification.

==> abstract.tex <==
We study an extension to the existential theory of integer arrays, which allows us to express properties that perform counting or accumulation. They include such statements as "the array length is correctly encoded in its first cell", or "the array contains equal number of minimal and maximal elements". These properties are orthogonal to those expressible in the quantified fragments of the theory of arrays, or in the theory of concatenation. We provide a decision procedure for the logic, and study its decidability and complexity. In particular, we show that it is NEXP complete, but under a natural restriction complexity reduces to NP. We also show that adding either a single universal quantifier or concatenation  leads to undecidability.

Our extension works by incorporating into the logic terms that fold some function over an array. We demonstrate that folding, a well-known concept from functional languages, allows us to concisely summarize loops that count or accumulate over arrays; such loops occur frequently in real-life programs. We provide a tool that is able to discharge proof obligations in our logic, and demonstrate on practical examples that our logic and decision procedure opens a new class of problems to formal methods such as symbolic testing or verification.

==> preliminaries.tex <==
 We assume familiarity with the standard syntax and terminology of many-sorted first-order logics. We use vector notation: $\vec{v} = (v_1,\ldots,v_n)$ denotes an ordered sequence of terms. For two vectors $\vec{u}$ and $\vec{v}$, we write their concatenation as $\vec{u}\vec{v}$.

%\subsection{Notation}
%
%For notational convenience, we use vector notation:
%$\vec{w} = (w_1,\ldots,w_n)$ to denote an ordered sequence of terms.
%Given two vectors $\vec{w}$ and $\vec{v}$, we denote their
%concatenation as $\vec{w}\vec{v}$.
%
%A formula $\vec{x}=\vec{y}$ means that the sizes of vectors $\vec{x}$
%and $\vec{y}$, as well as the corresponding elements $x_i$ and $y_i$,
%are equal.
%
%Everywhere in the paper, if not stated otherwise, we use the following
%convention: $a$, $b$ are array variables; $i$, $j$ are integer
%variables; $m$, $n$ are integer constants.

\subsection{Theory of Arrays}


%A set $\mathcal{Q}$ of strings over $\{\exists,\forall\}$ denotes the $Q$-fragment of a first-order theory: all formulas in the fragment are of the form $\mathcal{d} \partial_1 v_1 \cdots \partial_n \varphi$, where $\varphi$ is a quantifier-free formula.

Within this paper we consider the domains of arrays, array
indices, and array elements to be $\Ab = \Zb^*$,
$\Nb = \{\,0,1,\ldots \,\}$, and $\Zb = \{\,\ldots,-1,0,1,\ldots \,\}$
respectively.

Presburger arithmetic has the the signature
$\Sigma_{\mathbb{Z}} = \{\,0,1,+,<\,\}$; we use it for array indices
and elements, as well as other arithmetic assertions, possibly with
embedded array terms.
%$\Sigma_{\mathbb{Z}} = \{\,0,1,+,-,=,<\,\}$
We write $\true$ and $\false$ to denote a valid and an unsatisfiable Presburger formula, respectively.

The theory of integer-indexed arrays extends Presburger arithmetic
with functions \var{read}, and \var{write}, and has the signature
$\Sigma_{A} = \Sigma_{\mathbb{Z}} \cup \{\,\cdot[\cdot],\cdot\{\cdot
\leftarrow \cdot\}\, \}$.
The \var{read} function $a[i]$ returns the $i$-th element of array
$a$, and the \var{write} function $a\{i \leftarrow x\}$ returns array $a$ where the $i$-th element is replaced by $x$. These functions should satisfy the \emph{read}-over-\emph{write} axioms as described by McCarthy \cite{McCarthy62}.

%\subsection{Counter Machines}
%\label{subsec:cm}
%
%A counter machine is a finite state automaton extended by a vector
%$\ctrv= (\ctr_1, \ldots, \ctr_k)$ of $k$ counters. Every counter in
%$\ctrv$ stores a non-negative value, and a counter machine can compare
%it to constant, and increment/decrement its value by a constant. If,
%due to a decrement, the value of a counter drops below zero, then
%the behavior of the counter machine is undefined.
%
%Consider a vector $\ctrv = (\ctr_1, \ldots, \ctr_k)$ of counters, and a set $X$ of integer variables.
%An \emph{atomic counter constraint} is a formula of the form
%$\ctr_i \approx c$ or $\ctr_i \approx x$, where $c\in \Nb$, $x\in X$,
%and $\approx \in \{<,\le,>,\ge,=, \ne\}$.  A \emph{counter constraint}
%is either a conjunction of $n\geq 1$ atomic counter constraints, or the formula $\true$.
%We write $\cc_k(X)$ to denote the set of all counter constraints over variables in $X$ and
%counters in $\ctrv$. Notation $\cc_k(\emptyset)$ implies that
%counters are only compared to constants.
%
%\begin{definition}
%\label{def:cm}
%  A $k$-\emph{counter machine} is a tuple
%  $\scm = (\ctrv, \alphabet, \states, \tr, \init)$, where
%%\begin{itemize}
%%\item
% $\ctrv= (\ctr_1, \ldots, \ctr_k)$ is a vector of $k$ counter variables,
%%\item 
%$\alphabet$ is a finite set alphabet symbols,
%%\item 
%$\states$ is a finite set of states,
%%\item 
%$\tr \subseteq \states\times \cc_k(\emptyset)\times \alphabet\times\states\times\Zb^k$ is a transition relation,
%%\item
%and $\init \in \states$ is the initial state. A transition $(q_1,c,\alpha,q_2,\vec{\kappa}) \in \delta$ moves the counter machine from state $q_1$ to $q_2$ if the counters satisfy the constraint $c$ and the input symbol $\alpha$ is read; the counters are incremented by $\vec{\kappa}$.
%%\end{itemize}
%\end{definition}
%%
%%\begin{definition}
%%\label{def:scm}
%%  A $k$-\emph{counter machine} is a tuple
%%  $\scm = (\ctrv, \alphabet, \states, \tr, \init)$, where
%%\begin{itemize}
%%\item
%% $\ctrv= (\ctr_1, \ldots, \ctr_k)$ is a vector of $k$ counter variables,
%%\item $\alphabet$ is a finite set alphabet symbols,
%%\item $\states$ is a finite set of states,
%%\item $\tr$ is a transition relation, which is a finite subset of 
%%  $\states\times \cc_k(\emptyset)\times \alphabet\times\states\times\Zb^k$
%%\item $\init \in \states$ is the initial state.
%%\end{itemize}
%%\end{definition}
%
%% A \emph{configuration} of $\cm$ is a tuple
%% $\conf=(q, \vec{v})\in \states\times \Nb^k$.  The machine can make a
%% transition from configuration $\conf=(q, \vec{v})$ to
%% $\conf'=(p, \vec{u})$ on symbol $\alpha\in \alphabet$, written as
%% $\conf\xrightarrow{\alpha}\conf'$, if there is a transition
%% $(q, C, \alpha, q, \vec{w})\in \tr$, such that
%% $\vec{u} = \vec{v} + \vec{w}$ and $\vec{v}$ satisfies every counter
%% constraint in $C$. A path $\pi$ in a $\cm$ is a sequence
%% $\pi = \conf_0 \xrightarrow{\alpha_1} \ldots \xrightarrow{\alpha_n} \conf_n$,
%% such that $\conf_0=(\init, \cdot)$. A word $w\in \Sigma^*$ is accepted
%% by $\cm$ if there exists a path $w = \alpha_0\cdots\alpha_n$.
%
%
%
%A machine is called \emph{deterministic} if $\tr$ is functional, and
%\emph{one-way} if the tape head never moves back.  A counter machine
%makes a \emph{reversal} if it makes an alternation between
%non-increasing and non-decreasing some counter.  A machine is
%\emph{reversal-bounded} if there exists a constant $c\geq 0$ such
%that on all accepting runs every counter makes at most $c$ reversal.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> related.tex <==
\begin{enumerate}
\item Comparison to other array logics
\item About concolic testing and symbolic execution
\end{enumerate}


